EviHunter: Identifying Digital Evidence in the Permanent Storage of Android Devices via Static Analysis

Crimes, both physical and cyber, increasingly involve smartphones due to their ubiquity. Therefore, digital evidence on smartphones plays an increasingly important role in crime investigations. Digital evidence could reside in the memory and permanent storage of a smartphone. While we have witnessed significant progresses on memory forensics recently, identifying evidence in the permanent storage is still an underdeveloped research area. Most existing studies on permanent-storage forensics rely on manual analysis or keyword-based scanning of the permanent storage. Manual analysis is costly, while keyword matching often misses the evidentiary data that do not have interesting keywords. In this work, we develop a tool called EviHunter to automatically identify evidentiary data in the permanent storage of an Android device. There could be thousands of files on the permanent storage of a smartphone. A basic question a forensic investigator often faces is which files could store evidentiary data. EviHunter aims to answer this question. Our intuition is that the evidentiary data were produced by apps; and an app's code has rich information about the types of data the app may write to a permanent storage and the files the data are written to. Therefore, EviHunter first pre-computes an App Evidence Database (AED) via static analysis of a large number of apps. The AED includes the types of evidentiary data and files that store them for each app. Then, EviHunter matches the files on a smartphone's permanent storage against the AED to identify the files that could store evidentiary data. We evaluate EviHunter on benchmark apps and 8,690 real-world apps. Our results show that EviHunter can precisely identify both the types of evidentiary data and the files that store them.

==> realworldAppResult_table.tex <==
\begin{table}[]
\centering
\caption{Statistics of our analysis results for the 30,586 real-world apps.}
\label{table:realworldAppStat}

\bgroup
\def\arraystretch{1.5}%

\begin{tabular}{|c|c|}
\hline
Saved Evidence Type & Number of Apps \\ \hline
Device ID           & 1629           \\ \hline
Location            & 2494           \\ \hline
Contacts            & 0              \\ \hline
Time                & 6225           \\ \hline
Browsing History    & 2273           \\ \hline
Text Input          & 5307           \\ \hline
\end{tabular}%

\egroup

\end{table}


==> realworldEvidenceResult_table.tex <==
\begin{table*}[]
\caption{Analysis results for each type of evidentiary data on the 30,586 real-world apps. The column ``Static'' indicates the number of static file paths; the column ``Dynamic'' indicates the number of dynamic file paths; and the column ``App'' indicates the number of apps.}
%Since the logging system stores log messages in kernel buffers that are not individual files, we count the number of apps only.
\label{table:realworldEvidenceResult}
\vspace{2mm}

\centering
\def\arraystretch{1.2}%  1 is the default, row padding
\makebox[\linewidth]{\scriptsize%

\begin{threeparttable}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{3}{*}{File Type} & \multicolumn{12}{c|}{ Evidence Type} \\ \cline{2-13} 

& \multicolumn{3}{c|}{Location} & \multicolumn{3}{c|}{Time} & \multicolumn{3}{c|}{Visited URL} & \multicolumn{3}{c|}{Text Input} \\ \cline{2-13} 
& Static & Dynamic & App & Static & Dynamic & App & Static & Dynamic & App & Static & Dynamic & App \\ \hline

Text File  & 167 & 10 & 173 & 1019 & 142 & 1017 & 130 & 3 & 132 & 1940 & 35 & 1744 \\ \hline

Binary File & 16 & 1 & 17 & 109 & 3 & 73  & 30 & 0 & 18 & 103 & 18 & 88 \\ \hline

SQLite Database & 192 & 0 & 189 & 399 & 0 & 373  & 252 & 0 & 252 & 1417 & 0 & 1037 \\ \hline

SharedPreferences File & 362 & 0 & 236 & 2678 & 1 & 2401 & 81 & 0 & 81 & 1617 & 1 & 1516 \\  \hline

%Logging System & - & - & 1782 & - & - & 2555 & - & - & 1685 & - & - & 966 \\ \hline

Total & 737 & 11 & 615 & 4205 & 146 & 3864 & 493 & 3 & 483 & 5077 & 54 & 4385 \\  \hline

\end{tabular}

%\hspace{2cm}
%\begin{tablenotes}
%	\item [1] Since logging system stores messages in kernel buffers that are not individual files, we count the number of apps only.
%\end{tablenotes}

\end{threeparttable}}


\end{table*}

